The Complexity of Robot Games on the Integer Line

In robot games on Z, two players add integers to a counter. Each player has a finite set from which he picks the integer to add, and the objective of the first player is to let the counter reach 0. We present an exponential-time algorithm for deciding the winner of a robot game given the initial counter value, and prove a matching lower bound.

==> eptcsdata.tex <==
\providecommand{\firstpage}{132}
\providecommand{\publicationstatus}{L. Bortolussi and H. Wiklicky (Eds.): QAPL 2013\\
EPTCS 117, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.117.9}{10.4204/EPTCS.117.9}}

